Predicting Postoperative Intraocular Lens Dislocation in Cataract Surgery via Deep Learning

A critical yet unpredictable complication following cataract surgery is intraocular lens dislocation. Postoperative stability is imperative, as even a tiny decentration of multifocal lenses or inadequate alignment of the torus in toric lenses due to postoperative rotation can lead to a significant drop in visual acuity. Investigating possible intraoperative indicators that can predict post-surgical instabilities of intraocular lenses can help prevent this complication. In this paper, we develop and evaluate the first fully-automatic framework for the computation of lens unfolding delay, rotation, and instability during surgery. Adopting a combination of three types of CNNs, namely recurrent, region-based, and pixel-based, the proposed framework is employed to assess the possibility of predicting post-operative lens dislocation during cataract surgery. This is achieved via performing a large-scale study on the statistical differences between the behavior of different brands of intraocular lenses and aligning the results with expert surgeons' hypotheses and observations about the lenses. We exploit a large-scale dataset of cataract surgery videos featuring four intraocular lens brands. Experimental results confirm the reliability of the proposed framework in evaluating the lens' statistics during the surgery. The Pearson correlation and t-test results reveal significant correlations between lens unfolding delay and lens rotation and significant differences between the intra-operative rotations stability of four groups of lenses. These results suggest that the proposed framework can help surgeons select the lenses based on the patient's eye conditions and predict post-surgical lens dislocation.

==> 08_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Negin_Ghamsarian.jpeg}}]{Negin Ghamsarian} is a postdoctoral researcher at the "AI for Medical Imaging" Laboratory in the Department of Medicine at the University of Bern (Switzerland). She obtained her Ph.D. in computer science in 2021 from Klagenfurt University (Austria), where she also served as a research assistant on the project "Deep-Learning-Assisted Analysis of Surgical Videos" from 2019. Her research interests revolve around the application of deep learning techniques, including supervised learning, semi-supervised learning, and unsupervised domain adaptation, for action recognition in surgical videos and  semantic segmentation in medical images.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/doris_putzgruber.jpg}}]{Doris Putzgruber-Adamitsch} is board certified senior ophthalmologist at the department of ophthalmology at the Klinikum Klagenfurt. Besides extensive clinical surgical expertise, her main research focus is on the use of digitalized surgical videos and their use in teaching as well as evaluation of adverse events. 
\end{IEEEbiography}

 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/StephanieSarny.jpg}}]{Stephanie Sarny} was senior ophthalmologist at the department of ophthalmology at the Klinikum Klagenfurt. She holds a Ph.D. in medical science and has authored multiple research papers in peer-reviewed journals. Her research focuses on various topics in epidemiologic medical studies and different aspects of ophthalmic surgical video analysis.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Sznitman-1.png}}]{Raphael Sznitman} graduated in cognitive systems from the University of British Columbia (Canada) in 2007. He received his Ph.D. in computer science from Johns Hopkins University (USA) in 2011. He was then a postdoctoral fellow at the École Polytechnique Fédérale de Lausanne (Switzerland), where he worked in the computer vision laboratory. In 2015, he joined the faculty of the ARTORG Center at the University of Bern (Switzerland), where he is now a full professor in AI for Medical Imaging and the director of the ARTORG Center for Biomedical Engineering. His research interests are primarily in computational vision, probabilistic methods, and statistical learning, applied to applications in medical imaging.

\end{IEEEbiography}

 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/schoeffmann_klaus_resized-q.jpg}}]{Klaus Schoeffmann} is an associate professor at the Institute of Information Technology (ITEC) at Klagenfurt University, Austria. His research focuses on video content understanding (in particular medical/surgery videos), multimedia retrieval, interactive multimedia, and applied deep learning. He has co-authored more than 100 publications on various topics in multimedia, inclusive of many works on different aspects of medical video analysis. He has co-organized several international conferences, workshops, and special sessions in the field of multimedia. He is a member of the IEEE and the ACM, and a regular reviewer for international conferences and journals in the field of multimedia.
\end{IEEEbiography}

 

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Yosuf_El-Shabrawi2.jpeg}}]{ Yosuf El-Shabrawi} is the head of the department of ophthalmology at the Klinikum Klagenfurt. He is an assoc. Professor of Ophthalmology at the Department of Ophthalmology at the Medical University Graz as well as a lecturer at Medical University Vienna. His research focuses mainly on the various aspects of immunologic disorders in the eye as well as the use of machine learning in evaluating ophthalmic surgical videos. Dr. El-Shabrawi authored more than 100 papers published in peer-reviewed journals. 
\end{IEEEbiography}

==> Algorithms/LensID.tex <==




==> LensID.tex <==



